Linear Time Sinkhorn Divergences using Positive Features

Although Sinkhorn divergences are now routinely used in data sciences to compare probability distributions, the computational effort required to compute them remains expensive, growing in general quadratically in the size $n$ of the support of these distributions. Indeed, solving optimal transport (OT) with an entropic regularization requires computing a $n\times n$ kernel matrix (the neg-exponential of a $n\times n$ pairwise ground cost matrix) that is repeatedly applied to a vector. We propose to use instead ground costs of the form $c(x,y)=-\log\dotp{\varphi(x)}{\varphi(y)}$ where $\varphi$ is a map from the ground space onto the positive orthant $\RR^r_+$, with $r\ll n$. This choice yields, equivalently, a kernel $k(x,y)=\dotp{\varphi(x)}{\varphi(y)}$, and ensures that the cost of Sinkhorn iterations scales as $O(nr)$. We show that usual cost functions can be approximated using this form. Additionaly, we take advantage of the fact that our approach yields approximation that remain fully differentiable with respect to input distributions, as opposed to previously proposed adaptive low-rank approximations of the kernel matrix, to train a faster variant of OT-GAN \cite{salimans2018improving}.

==> sections/ack.tex <==
\section*{Acknowledgements}
This work was funded by a "Chaire d’excellence de l’IDEX Paris Saclay".

==> sections/sec4_old.tex <==
\section{Approximation properties of Positive Features}
Let us now consider kernels which can be written for all $x,y\in\mathcal{X}$ as
\begin{align}
\label{eq:general}
k(x,y)=\int_{u\in\mathcal{U}} \varphi(x,u)^T\varphi(y,u) d\rho(u)
\end{align}
where $\mathcal{U}$ is a metric space, $\rho$ is a probability measure on $\mathcal{U}$ and
$\varphi:\mathcal{X}\times\mathcal{U}\rightarrow (\mathbb{R_{+}^{*}})^p$ such that for all $x\in\mathcal{X}$, $u\in\mathcal{U}\rightarrow \Vert\varphi(x,u)\Vert_2$ is square integrable (for the measure $d\rho$). In fact, we will see in the following that for some usual cost functions $c$, the Gibbs kernel associated $k(x,y)=\exp(-\varepsilon^{-1} c(x,y))$ admits such a decomposition. To obtain a finite-dimensional representation, one can approximate the integral with a weighted finite sum. Let $r\geq 1$ and  $\theta:=(u_1,...,u_r)\in\mathcal{U}^r$ from which we can define the following positive feature map 
$$\varphi_{\mathbf{\theta}}(x) \defeq\frac{1}{\sqrt{r}}\left(\varphi(x,u_1),...,\varphi(x,u_r)\right)\in\mathbb{R}^{p\times r}$$
and obtain an approximation of the kernel $k$ defined as $k_{\theta}(x,y)\defeq\langle \varphi_{\mathbf{\theta}}(x),\varphi_{\mathbf{\theta}}(y)\rangle$. In the next section, our goal is to control uniformly the relative error between these two kernels. 


\subsection{Kernel Approximation via Random Features}
To simplify the notations assume that $n=m$. Here we show with high probability that for all $(x,y)\in\mathcal{X}\times \mathcal{X}$,
\begin{align}
\label{eq:goal-RFF}
    (1-\delta)k(x,y)\leq k_{\theta}(x,y)\leq (1+\delta)k(x,y)
\end{align}
for an arbitrary $\delta>0$ as soon as the number of random features $r$ is large enough. See Appendix~\ref{proof:ratio-RFF} for the proof.

\todo{il manque une phrase qui explique cette prop pour m. tout le monde, et qui motive son importance.}

\begin{prop}
\label{lem:ratio-RFF}
Let $\mathcal{X}\subset \mathbb{R}^d$ compact, $n\geq 1$,  $\mathbf{X}= \{x_1,...,x_n\}$ and $\mathbf{Y}= \{y_1,...,y_n\}$ such that $\mathbf{X},\mathbf{Y}\subset\mathcal{X}$,  $\delta>0$ and $k$ kernel on $\mathcal{X}$ defined as in (\ref{eq:general}) such that for all $x,y\in\mathcal{X}$, $k(x,y)>0$. Let also $r\geq 1$, $u_1,...,u_r$ drawn randomly from $\rho$ and let us assume that there exists $K>0$ such that:
\begin{align}
\label{eq:assump:ratio}
    K:=\sup_{x,y\in\mathcal{X}}\sup_{u\in\mathcal{U}}\left|\frac{\varphi(x,u)^T\varphi(y,u)}{k(x,y)}\right|<+\infty.
\end{align}
First we have
\begin{align*}
\label{eq:finit-RFF}
\mathbb{P}\left(\sup_{(x,y)\in\mathbf{X}\times\mathbf{Y}}\left |\frac{k_{\theta}(x,y)}{k(x,y)}-1\right|\geq \delta\right)\leq 2 n^2\exp\left(-\frac{r \delta^2}{2 K^2}\right)
\end{align*}
and if we assume in addition that there exists $\kappa>0$ such that for all $x,y\in\mathcal{X}$, $k(x,y)\geq\kappa$ and that  $\varphi$ is differentiable such that
\begin{align*}
    V:=\sup_{x\in\mathcal{X}}\mathbf{E}_{\rho}\left(\Vert \nabla_x\varphi(x,u)\Vert^2\right)<+\infty
\end{align*}
we have that
\begin{align*}
\mathbb{P}\left(\sup_{(x,y)\in\mathcal{X}\times\mathcal{X}}\left |\frac{k_{\theta}(x,y)}{k(x,y)}-1\right|\geq \delta\right)\leq \frac{(\kappa^{-1}D)^2 C_{K,V,r}}{\delta^2}\exp\left(-\frac{r\delta^2}{2K^2(d+1)}\right)
\end{align*}
where $C_{K,V,r} = 2^9 K(4+K^2/r)V \sup\limits_{x\in\mathcal{X}}k(x,x)$, and $D=\sup\limits_{(x,y)\in\mathcal{X}\times\mathcal{X}}\Vert(x,y)\Vert_2$.
\end{prop}

\todo{p ê dire que c'est une remarque? et la référer dans l'intro pour clarifier la dif?}
\paragraph{Ratio Approximation.} The uniform bounds obtained to control of the ratio between the approximation and the kernel gives naturally a control of the form eq.(\ref{eq:goal-RFF}). In comparison, in \cite{rahimi2008random}, the authors obtain a uniform bound on their difference which leads to a control in high probability of the form 
\begin{align}
    k(x,y)-\tau\leq k_{\theta}(x,y)\leq k(x,y)+\tau
\end{align}
where $\tau$ is a decreasing function with respect to $r$. To be able to recover eq.(\ref{eq:goal-RFF}) from the above control, on may consider the case when $\tau=\inf\limits_{x,y\in\mathbf{X}\times\mathbf{Y}}k(x,y)\delta$ which in some cases may considerably increases the number of of random features $r$ needed to ensure the result with at leat the same probability. For example if the kernel is the Gibbs kernel associated to a cost function $c$, then  $\inf\limits_{x,y\in\mathbf{X}\times\mathbf{Y}}k(x,y)=\exp(-\Vert C\Vert_\infty/\varepsilon)$.

% \paragraph{Ratio Approximation.} Let us assume here that $p=1$ for simplicity. The main goal is to obtain a control of $k_{\theta}$ of the form eq.(\ref{eq:goal-RFF}) with a minimum number of random features $r$. In the lemma above, we obtain such a result with a probability of at least $1-2 n^2\exp\left(-\frac{r \delta^2}{2 K^2}\right)$ where $r$ is the number of random features and $K$ is defined as 
% \begin{align*}
%  K:=\sup_{u\in\mathcal{U}}\sup_{ (x,y)\in\mathbf{X}\times\mathbf{Y}}\left|\frac{\varphi(x,u)\varphi(y,u)}{k(x,y)}\right|
% \end{align*}
% and is assumed to be finite. Now assume that there exists $C$ such that for all $(x,y)\in\mathbf{X}\times \mathbf{Y}$ and $u\in\mathcal{U}$,  $$|\varphi(x,u)\varphi(y,u)|\leq C.$$
% Then by defining
% \begin{align*}
%     K'=\sup_{u\in\mathcal{U}}\sup_{ (x,y)\in\mathbf{X}\times\mathbf{Y}}\left|\varphi(x,u)\varphi(y,u)\right|
% \end{align*}
% an analogue proof gives that with a probability of at least $1-2 n^2\exp\left(-\frac{r \tau^2}{2 K'^2}\right)$ for all $(x,y)\in\mathbf{X}\times\mathbf{Y}$ (\cite{rahimi2008random})
% \begin{align}
%     k(x,y)-\tau\leq k_{\theta}(x,y)\leq k(x,y)+\tau
% \end{align}
% To be able to recover eq.(\ref{eq:goal-RFF}) from the above control, we need to take  $\tau=\inf\limits_{x,y\in\mathbf{X}\times\mathbf{Y}}k(x,y)\delta$ and by denoting $K_1=\frac{K'}{\inf\limits_{x,y\in\mathbf{X}\times\mathbf{Y}}k(x,y)}$ we obtain that with a probability of at least $1-2 n^2\exp\left(-\frac{r \delta^2}{2 K_1^2}\right)$ for all $(x,y)\in\mathbf{X}\times\mathbf{Y}$
% \begin{align*}
%     (1-\delta) k(x,y) \leq k_{\theta}(x,y)\leq (1+\delta)k(x,y)
% \end{align*}
% Therefore the number of random features needed to guarantee eq.(\ref{eq:goal-RFF}) from a control between the difference of the two kernels with at least a probability $1-\delta$ has to be larger than $\left(\frac{K_1}{K}\right)^2$ times the number of random features needed from the control of Proposition \ref{lem:ratio-RFF} to guarantee eq.(\ref{eq:goal-RFF}) with at least the same probability $1-\delta$. But we always have that
% \begin{align*}
%     K=\sup_{u\in\mathcal{U}}\sup_{ (x,y)\in\mathbf{X}\times\mathbf{Y}}\left|\frac{\varphi(x,u)\varphi(y,u)}{k(x,y)}\right|\leq \frac{\sup\limits_{u\in\mathcal{U}}\sup\limits_{ (x,y)\in\mathbf{X}\times\mathbf{Y}}\left|\varphi(x,u)\varphi(y,u)\right|}{\inf\limits_{x,y\in\mathbf{X}\times\mathbf{Y}}k(x,y)}=K_1
% \end{align*}
% and in some cases the ratio $\left(\frac{K_1}{K}\right)^2$ can be huge. Indeed, as we will see in the following, for the Gaussian kernel,
% $$k(x,y)=\exp(-\varepsilon^{-1}\Vert x-y\Vert_2^2)$$
% there exists $\varphi$ and $\mathcal{U}$ such that for all $x,y$ and $u\in\mathcal{U}$:
% \begin{align*}
% \varphi(x,u)\varphi(y,u)=k(x,y)h(u,x,y)
% \end{align*}
% where for all $(x_0,y_0)\in\mathbf{X}\times\mathbf{Y}$,
% $$\sup\limits_{u\in\mathcal{U}}|h(u,x_0,y_0)|=\sup\limits_{u\in\mathcal{U}}\sup\limits_{ (x,y)\in\mathbf{X}\times\mathbf{Y}}|h(u,x,y)|.$$ 
% Therefore by denoting  $M=\sup\limits_{ (x,y)\in\mathbf{X}\times\mathbf{Y}}\Vert x-y\Vert_2$ and $m=\inf\limits_{ (x,y)\in\mathbf{X}\times\mathbf{Y}}\Vert x-y\Vert_2$ , we obtain that
% \begin{align*}
% \left(\frac{K_1}{K}\right)^2=\left(\frac{\sup\limits_{x,y\in\mathbf{X}\times\mathbf{Y}}k(x,y)}{\inf\limits_{x,y\in\mathbf{X}\times\mathbf{Y}}k(x,y)}\right)^2=\exp\left(2\varepsilon^{-1}[M^2-m^2]\right)
% \end{align*}


\subsection{Examples}
Here we provides examples of some usual kernels $k$ that admits a decomposition of the form eq.(\ref{eq:general}) and we show that the assumptions of Proposition \ref{lem:ratio-RFF} are  satisfied. Moreover it happens \MC{pas très clair ce "it happens"?} that these kernels may be the Gibbs kernels $k(x,y)=\exp(-\varepsilon^{-1} c(x,y))$  associated to some usual cost functions $c$. 
\MC{je me demande s'il ne faut pas séparer/distinguer les exemples directs, constructifs, des approximations de l'existant (e.g. Gaussien)}
\textbf{Transport on the Positive Sphere.} \MC{je pense qu'il faut dire que qq part c'est un peu un linear kernel} Defining a cost as the log of a dot-product as described in \eqref{eq:cost} has already played a role in the recent OT literature. These references do not, however, consider such cost functions for practical considerations, as we do in this paper.~\citet{OLIKER2007600} defines a cost $c$ on the sphere $\mathbb{S}^d$, as $c(x,y)=-\log x^Ty, \text{if } x^Ty>0$, and $\infty$ otherwise. The cost is therefore finite whenever two normal vectors share the same halfspace, and infinite otherwise. A variant of that cost  $-\log(1-x^Ty)$ also plays an important role in the reflector problem~\citep{glimm2003optical}, whose goal is to design a reflector able to reflect an incoming source of light in such a way that it matches a desired illumination. 
In several concurrent works,~\citet{LieroMielkeSavareShort}, \citet{2017-chizat-focm} and~\citet{kondratyev2016new} have considered the cost $c(x,y)= - \log (\cos (d(x,y)\wedge \pi/2)$ where $d$ is any metric. Note that when the metric is the geodesic distance on the sphere, $d(x,y)=\arccos(x^Ty)$ one then recovers exactly~\citeauthor{OLIKER2007600}'s cost. See Appendix \ref{sec:OT-sphere} for an illustration. %When restricting the feature maps $\varphi_\theta$ to take values in the positive orthant, not necessarily in the sphere, one obtains by design a non-normalized ``self-cost'' $c(x,x)=-\log(\|\varphi_\theta(x)\|^2)$ that may be positive (low norms) or negative (high norms). 
% Note that unlike other formulations of regularized transport, there is no regularization parameter so to speak in this case, since these kernels does not have a bandwidth parameter that can be tuned. 

\textbf{Arc-cosine Kernels.} Arc-cosine kernels have been considered in several works, starting notably from~\citep{NIPS2000_1790}, \citep{NIPS2009_3628}
and~\citep{JMLR:v18:14-546}. The main idea behind arc-cosine kernels is to define positive maps for vectors $x,y$ in $\mathbb{R}^d$ using the signs (or higher exponent) of random projections $\mu= \mathcal{N}(0,I_d)$
$$
k_s(x,y) = \int_{\mathbb{R}^d}\Theta_s(u^T x) \Theta_s(u^T y)d\mu(u)
$$
where $\Theta_s(w) = \sqrt{2}\max(0,w)^s$ is a rectified polynomial function, and show that these integrals coincide with kernels that only involve the norms and the angle between $x,y$,
$$k_s(x,y)= \frac{1}{\pi}\|x\|^s\|y\|^s J_s\left(\arccos\left(\frac{x^T y}{\|x\|\|y\|}\right)\right),$$
where $$J_s(u)=(-1)^s(\sin u)^{2s+1}\left(\frac{1}{\sin u}\tfrac{\partial}{\partial \theta}\right)^s\left(\frac{\pi-u}{\sin u}\right).$$ 
To be able to define a cost function from such kernels, we need to ensure that the kernels $k_s$ take value in $\mathbb{R}^{*}_+$. In the following lemma, we show that one can build a perturbed version of $k_s$ which admits a decomposition of the form eq.(\ref{eq:general}) that satisfies the assumption of Proposition \ref{lem:ratio-RFF}. See Appendix \ref{proof:lemma_arccos} for the proof.
\begin{lemma}
\label{lem:decomp-arccos}
Let $d\geq 1$, $s\geq 0$, $\kappa>0$ and $k_{s,\kappa}$ be the perturbed arc-cosine kernel on $\mathbb{R}^d$ defined as for all $x,y\in\mathbb{R}^d$, $ k_{s,\kappa}(x,y) = k_s(x,y) + \kappa$. Let also $\sigma>1$, $\rho=\mathcal{N}\left(0,\sigma^2\text{Id}\right)$ and let us define for all $x,u\in\mathbb{R}^d$ the following map:
\begin{align*}
    \varphi(x,u)=\left(\sigma^{d/2}\sqrt{2}\max(0,u^T x)^s\exp\left(-\frac{\Vert u\Vert^2}{4}\left[1-\frac{1}{\sigma^2}\right]\right),\sqrt{\kappa}\right)^T 
\end{align*}
Then for any $x,y\in\mathbb{R}^d$ we have:
\begin{align*}
k_{s,\kappa}(x,y)&=\int_{u\in\mathbb{R}^d} \varphi(x,u)^T\varphi(y,u) d\rho(u)
\end{align*}
Moreover we have for all $x,y\in\mathbb{R}^d$ $k_{s,\kappa}(x,y)\geq \kappa>0$ and for any compact $\mathcal{X}\subset\mathbb{R}^d$ we have:
\begin{align*}
\sup_{u\in\mathbb{R}^d}\sup_{ (x,y)\in\mathcal{X}\times\mathcal{X}}\left|\frac{\varphi(x,u)\varphi(y,u)}{k(x,y)}\right|<+\infty\quad \text{and} \quad    \sup_{x\in\mathcal{X}}\mathbf{E}(\Vert \nabla_x\varphi\Vert_2^2)<+\infty
\end{align*}
\end{lemma}



\textbf{Gaussian kernel.} The Gaussian kernel is in fact an important example as it is both a very widely used kernel on its own and its cost function associated is the $\ell_2$ square metric. In the following lemma, we show that the Gaussian kernel admits a decomposition of the form eq.(\ref{eq:general}) that satisfies the assumption of Proposition \ref{lem:ratio-RFF}. See Appendix \ref{proof:lemma_gaussian} for the proof.
\begin{lemma}
\label{lem:decomp-RBF}
Let $d\geq 1$, $\varepsilon>0$ and $k$ be the kernel on $\mathbb{R}^d$ such that for all $x,y\in\mathbb{R}^d$
\begin{align*}
    k(x,y)=e^{-\Vert x-y\Vert_2^{2}/\varepsilon}.
\end{align*}
Let $R>0$, $q=\frac{R^2}{2\varepsilon d W_0\left(R^2/\varepsilon d\right)}$ where $W_0$ is the Lambert function, $\sigma^2 = \frac{q\varepsilon}{4}$, $\rho=\mathcal{N}\left(0,\sigma^2\text{Id}\right)$ and let us define for all $x,u\in\mathbb{R}^d$ the following map:
\begin{align*}
    \varphi(x,u)&=(2q)^{d/4}\exp\left(-2\varepsilon^{-1} \Vert x-u\Vert^2_2\right)\exp\left(\frac{\varepsilon^{-1}\Vert u\Vert_2^2}{\frac{1}{2}+\varepsilon^{-1} R^2}\right)
\end{align*}
Then for any $x,y\in\mathbb{R}^d$ we have:
\begin{align*}
k(x,y)&=\int_{u\in\mathbb{R}^d} \varphi(x,u)\varphi(y,u) d\rho(u)
\end{align*}
Moreover for any $x,y\in \mathcal{B}(0,R)$ and for any $u\in\mathbb{R}^d$ we have $k(x,y)\geq \exp(-4\varepsilon^{-1} R^2)>0$ and
\begin{align*}
\left|\frac{\varphi(x,u)\varphi(y,u)}{k(x,y)}\right|\leq 2^{d/2+1} q^{d/2}.
\end{align*}
Finally we also have
\begin{align*}
    \sup_{x\in\mathcal{B}(0,R)}\mathbf{E}(\Vert \nabla_x\varphi\Vert_2^2)\leq  2^{d/2+3} q^{d/2} \left[(R/\varepsilon)^2+\frac{q}{4\varepsilon}\right]
\end{align*}
\end{lemma}


==> sections/sec5_old.tex <==
\section{Approximation of the Regularized Optimal Transport}
Here we present our main result \MC{si c'est le main result, il doit être annoncé avant} about the approximation of the ROT problem. In the following $k$ is a kernel which can be written eq.(\ref{eq:general}) and satisfies the assumptions of Proposition \ref{lem:ratio-RFF}.
% Let $\mathcal{X}\subset\mathbb{R}^d$ a compact set and $k$ a kernel on $\mathcal{X}\times\mathcal{X}$. Let us consider the following assumptions: \todo{enlever assumption et dire en une phrase le truck}
% \medbreak
% \textbf{Assumption 1}: 
% The kernel $k$ admits on $\mathcal{X}\times\mathcal{X}$ a decomposition of the form
% \begin{align}
% k(x,y)=\int_{u\in\mathcal{U}} \varphi(x,u)^T\varphi(y,u) d\rho(u)
% \end{align}
% where $\mathcal{U}$ is a metric space, $p\geq 1$, $\rho\in\mathcal{P}(\mathcal{U})$ and $\varphi:\mathcal{X}\times\mathcal{U}\rightarrow (\mathbb{R}_{+}^{*})^p$ such that for any $x\in\mathcal{X}$, $u\rightarrow\Vert \varphi(x,u)\Vert_2$ is a square integrable function.
% \medbreak
% \textbf{Assumption 2}:
% There exists a constant $K>0$ such that for all $x,y\in\mathcal{X}$:
% \begin{align}
%     \frac{\varphi(x,u)^T\varphi(y,u)}{k(x,y)}\leq K
% \end{align}
% \medbreak
% \textbf{Assumption 3}: 
% There exists a $\kappa>0$ such that for ally $x,y\in\mathcal{X}$, $k(x,y)\geq \kappa>0$.
% \medbreak
% \textbf{Assumption 4}: $\varphi$ is differentiable there exists $V>0$ such that:
% \begin{align}
%     \sup_{x\in\mathcal{X}}\mathbf{E}_{\rho}\left(\Vert \nabla_x\varphi(x,u)\Vert^2\right)\leq V
% \end{align}
% \medbreak
Let $\varepsilon>0$. Thanks to the positivity of the kernel $k$, we also define $c(x,y)\defeq -\varepsilon\log k(x,y)$ the cost function associated. In the following, we denote
$f\in\mathcal{O}(g)$ if $f\leq C g$ for a universal constant $C$ and $f\in\Omega(g)$ if $g\leq Q f$ for a universal constant $Q$. Let us now show the following theorem. See Appendix~\ref{proof:thm_approx_sin} for the proof.
\begin{thm}
\label{thm:result-sinkhorn-pos}
Let $\delta>0$ and $r\geq 1$. Then the Sinkhorn algorithm \ref{alg-sink} with inputs $\mathbf{K}_\theta:=(k_\theta(x_i,y_j))_{i,j=1}^n$, $a$ and $b$ outputs $(u_{\theta},v_{\theta})$ such that
    \begin{align*}
    |W_{\varepsilon,c_{\theta}}-\widehat{W}_{\varepsilon,c_\theta}|\leq \frac{\delta}{2}
\end{align*} 
in $\mathcal{O}\left(\frac{n\varepsilon r}{\delta}\left[\log\left(\frac{1}{c}\right)+Q_{\theta}\right]^2\right)$ algebric operations where
\begin{align*}
   c=\min\limits_{i,j}(a_i,b_j) \text{\quad and\quad}
   Q_{\theta}=\log\left(\frac{1}{\min_{i,j} 
k_{\theta}(x_i,y_j)}\right)
\end{align*}
Moreover let $\tau>0$, 
\begin{align}
\label{eq:number-feature}
 r\in\Omega\left(\frac{K^2}{\delta^2}\left[\min\left(d\varepsilon^{-1} \Vert C\Vert_{\infty}^2+d\log\left(\frac{KVD}{\tau\delta}\right),\log\left(\frac{n}{\tau}\right)\right)\right]\right)   
\end{align}
and $u_1,...,u_r$ drawn independently from $\rho$, then with a probability $1-\tau$, $Q_{\theta}\leq \varepsilon^{-1} \Vert C\Vert_{\infty}^2 +\log\left(2+\delta\varepsilon^{-1}\right)$ and it holds  
\begin{align}
  |W_{\varepsilon,c}-\widehat{W}_{\varepsilon,c_\theta}|\leq \delta
\end{align}
\end{thm}
% \begin{rmq}
% Assumptions 1 and 2 suffice to obtain a $\delta$-approximation of the ROT distance. Indeed in that case, if 
% \begin{align*}
%  r\in\Omega\left(\frac{K^2}{\delta^2}\left[\log\left(\frac{n}{\delta}\right)\right]\right)   
% \end{align*}
% then with a probability $1-\delta$, the Sinkhorn algorithm \ref{alg-sink} with inputs $\mathbf{K}_\theta$, $a$ and $b$ and after $\tilde{\mathcal{O}}\left(\frac{n}{\varepsilon\delta^3} \Vert C\Vert_{\infty}^4 K^2\right)$ algebraic operations, outputs $(u_{\theta},v_{\theta})$ such that
% \begin{align*}
%   |W_{\varepsilon,c}-\widehat{W}_{\varepsilon,c_\theta}|\leq \delta.
% \end{align*} 
% where the notation $\tilde{\mathcal{O}}(.)$ omits polylogarithmic factors depending on $R, D, \varepsilon,c, n$ and $\delta$.
% \end{rmq}
Therefore with a probability $1-\tau$, Sinkhorn algorithm \ref{alg-sink} with inputs $\mathbf{K}_\theta$, $a$ and $b$ output a $\delta$ approximation of the ROT distance in 
 $\tilde{\mathcal{O}}\left(\frac{n}{\varepsilon\delta^3} \Vert C\Vert_{\infty}^4 K^2\right)$ 
algebraic operation where the notation $\tilde{\mathcal{O}}(.)$ omits polylogarithmic factors depending on $R, D, \varepsilon,c, n$ and $\delta$.

It worth noting that for every $r\geq 1$ and $\theta$, Sinkhorn algorithm \ref{alg-sink} using kernel matrix $\mathbf{K}_{\theta}$ will converge towards an approximate solution of the ROT problem associated with the cost function $c_\theta$ in linear time thanks to the positivity of the feature maps used. Moreover, to ensure with high probability that the solutions obtained approximate an optimal solution for the ROT problem associated with the cost function $c$, we need, if the features are chosen randomly, to ensure a minimum number of them. In constrast such result may not possible in \cite{altschuler2018massively} as $r$ is the one obtained by the Nyström algorithm of \cite{musco2016recursive} which guarantee the positivity of the coefficients of the kernel matrix obtained and therefore needs a very high precision. 

\subsection{Accelerated methods}
\todo{Est-ce qu on laisse cela ou on dit une petite phrase comme quoi on a etudie le cas accelere en appendix aussi ?}
\cite{guminov2019accelerated} show that one can accelarated the Sinkhorn algorithm (see Appendix \ref{algo:acc-sinkhorn}) and obtain a $\delta$-approximation of the OT distance. For that purpose, \cite{guminov2019accelerated} introduce a reformulation of the dual problem (\ref{eq:dual-theta}) and obtain 
\begin{align}
\label{eq:dual-smooth}
W_{\varepsilon,c_{\theta}}=\sup_{\alpha,\beta} F_\theta(\alpha,\beta):=\varepsilon\left[\langle \alpha,a\rangle + \langle \beta,b\rangle -\log\left(\langle e^{\alpha},K_{\theta}e^{\beta}\rangle\right)\right]
\end{align}
which can be shown to be an $L$-smooth function (\cite{nesterov2005smooth}) where 
$L\leq 2\varepsilon^{-1}$. Applying our approximation scheme ot their algorithm leads to the following result. See proof in Appendix \ref{proof:thm-acc-sin}. 
\begin{thm}
\label{thm:result-acc-sinkhorn}
Let $\delta>0$ and $r\geq 1$. Then the Accelerated Sinkhorn algorithm \ref{algo:acc-sinkhorn} with inputs $\mathbf{K}_\theta$, $a$ and $b$ outputs $(\alpha_{\theta},\beta_{\theta})$ such that
    \begin{align*}
    |W_{\varepsilon,c_{\theta}}-F_\theta(\alpha_{\theta},\beta_{\theta})|\leq \frac{\delta}{2}
\end{align*} 
in $\mathcal{O}\left(\frac{nr}{\sqrt{\delta}} [\sqrt{\varepsilon^{-1}}A_\theta]\right)$ algebraic operations where $A_\theta=\inf\limits_{(\alpha,\beta)\in\Theta_{\theta}} \Vert (\alpha,\beta)\Vert_2$ and $\Theta_{\theta}$ is the set of optimal dual solutions of (\ref{eq:dual-smooth}). Moreover let $\delta>0$, 
\begin{align}
\label{eq:number-feature}
 r\in\Omega\left(\frac{K^2}{\delta^2}\left[\min\left(d\varepsilon^{-1} \Vert C\Vert_{\infty}^2+d\log\left(\frac{KVD}{\delta\delta}\right),\log\left(\frac{n}{\delta}\right)\right)\right]\right)   
\end{align}
and $u_1,...,u_r$ drawn independently from $\rho$, then with a probability $1-\delta$ it holds  
\begin{align}
  |W_{\varepsilon,c}-F_\theta(\alpha_{\theta},\beta_{\theta})|\leq \delta
\end{align}
\end{thm}
% \begin{rmq}
% It is worth noting that the Accelerated Sinkhorn algorithm can also be applied in combination with a Nyström approximation method as the one proposed in \cite{altschuler2018massively} and obtain similar improvments.
% \end{rmq}
\textbf{Illustrations.} In this experiment, we draw 40000 samples from two normal distributions respectively $\mu=\mathcal{N}(\mathbf{0},\sigma^2 \textbf{I}_d)$ where $d=2$ and $\sigma^2=10^{-1}$, and $\nu=\mathcal{N}(\mathbf{1}, \textbf{I}_d)$. Moreover the samples from $\nu$ has been scaled with the maximum norm of the samples, such that they live in the unit ball. In Figure \ref{fig:result_acc}, we plot the algebraic relative error\footnote{The algebraic relative errror considered in Figure \ref{fig:result_acc} is defined as $\text{RE}:=\frac{\widehat{\text{ROT}}-\text{ROT}}{\text{ROT}}$\MC{
éviter les footnotes}} with respect to the ground truth ROT distance ploted in the basis $100\%$ for different regularisations and compare the results obtained for our proposed method (\textbf{RF}) with the one proposed in \cite{altschuler2018massively} (\textbf{Nys}) and with the Sinkhorn algorithm (\textbf{Sin}) proposed in \cite{CuturiSinkhorn}. The number of random features (or rank) chosen varies from $100$ to $2000$. Given the fixed discrete distributions, we repeat for each regularisation 50 times the experiment with different seeds for both  (\textbf{RF} and \textbf{RF} methods and we plot the average of the results obtained. We observe that there is 3 regimes of interest. The first regime is when the regularisation is sufficiently large, which corresponds to the case when $\varepsilon=0.5$. Both \textbf{Nys} and \textbf{RF} methods obtain very high accuracy with order of magnitude faster than \textbf{Sin}. Note that \textbf{Nys} method achieves even better accuracy than \textbf{RF} method in this regime. Another regime of interest is when $\varepsilon=0.1$. In that case both \textbf{Nys} and \textbf{RF} reach the same very high accuracy at a given number of random features (or rank) with order of magnitude faster than \textbf{Sin}. However it is important to note that \textbf{Ny} method works only if the number of random features (or the rank) is sufficiently large, that is if $r\geq 1000$. Moreover, even if $r\geq 1000$, among the 50 trials done in this setting, only few converge ($\simeq 5$) for \textbf{Ny} method. This phenomena is repeated and amplified when $\varepsilon=0.05$ as the \textbf{Ny} method totally failed. However, the \textbf{RF} works totally well and provides with high accuracy an approximation of the ROT cost with order of magnitude faster than \textbf{Sin}. Finally, there is a regime, which is when $\varepsilon=0.01$, where all the methods failed. Indeed our proposed method performs poorly as the accuracy of the \textbf{RF} method is of order of $10\%$, the Nystrom method cannot be computed, and Sinkhorn algorithm may be too costly.

\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth, trim=0.5cm 1cm 0.5cm 1cm]{FastSinkhornGAN/img/plot_accuracy_ROT_relative_error_base_2_scale.pdf}
\caption{Accuracy vs Time.\label{fig:result_acc} \MC{les figures sont super. il faut maintenant trouver un moyen pour les agrandir, ainsi que les labels. il est envisageable de ne pas remettre le y-label sur tous les plots. il faut que les fonts soient plus grosses. peut être envisager une présentation en grille 2x2 qui serait sur les 3/5 de la colonne à droite en utilisant wrapfigure. Cette figure doit arriver bien avant la figure GAN. Peut on imaginer une autre appli synthétique? il faut que tu donnes un vrai titre (pas reg= ... , mais Regularization : ...}}
\end{figure}


% We add also in Table \ref{table:relative_acc} the relative errors of the different methods when the number of random features (or rank) is fixed to be 2000. Note that when $\varepsilon \leq 0.01$, the relative accuracy is large, and this is due to the fact that we only run the algorithms for 100 iterations. See Appendix \ref{fig:result_acc_high_reg}  for results when the regularisation gets larger.
% \begin{table*}[h!]
% \centering\small
% \begin{tabular}{lcccccc}
% Relative Error ($\%$) & $\varepsilon = 0.005$  &
% $\varepsilon = 0.01$  &
% $\varepsilon = 0.05$ &
% $\varepsilon = 0.1$ &
% $\varepsilon = 0.5$ &
% $\varepsilon = 1$  \\
% \hline
% Sinkhorn \cite{CuturiSinkhorn} & 186  &  91 &    0.13 & 0.045 &    0.029 &     0.027  \\
% Nystrom \cite{altschuler2018massively} &  NaN  &  NaN  &  NaN &     0.0072 &   0.0011 &     0.00099 \\
% Proposed Method &   178 &    84 &    0.13 &    0.071 &    0.046 &     0.039 \\
% \end{tabular}
% \caption{Relative Error. We plot the relative error with the ground truth after 100 iterations for each methods when $r=2000$.\label{table:relative_acc}}
% \label{Tab:exp3result}
% \end{table*}



